ICT: Image-Object Cross-Level Trusted Intervention for Mitigating Object Hallucination in Large Vision-Language Models

Despite the recent breakthroughs achieved by Large Vision Language Models (LVLMs) in understanding and responding to complex visual-textual contexts, their inherent hallucination tendencies limit their practical application in real-world scenarios that demand high levels of precision. Existing methods typically either fine-tune the LVLMs using additional data, which incurs extra costs in manual annotation and computational resources or perform comparisons at the decoding stage, which may eliminate useful language priors for reasoning while introducing inference time overhead. Therefore, we propose ICT, a lightweight, training-free method that calculates an intervention direction to shift the model's focus towards different levels of visual information, enhancing its attention to high-level and fine-grained visual details. During the forward pass stage, the intervention is applied to the attention heads that encode the overall image information and the fine-grained object details, effectively mitigating the phenomenon of overly language priors, and thereby alleviating hallucinations. Extensive experiments demonstrate that ICT achieves strong performance with a small amount of data and generalizes well across different datasets and models. Our code will be public.

==> main_result.tex <==

\begin{table}[t!]
  \caption{Results obtained using different forms of prompts on 10 accessible LLMs.}
  \label{main-result}
  \centering
    \scalebox{0.74}{
\begin{tabular}{ccccccccccc}
\toprule
    \multirow{2}{*}{Methods} & \multicolumn{2}{c}{Zero-shot w/o CoT} & \multicolumn{2}{c}{Zero-shot w/ CoT} & \multicolumn{2}{c}{Few-shot w/o CoT} & \multicolumn{2}{c}{Few-shot w/ CoT} & \multicolumn{2}{c}{Overall Performance} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}  \cmidrule(lr){8-9} \cmidrule(lr){10-11}
                         & Accuracy          & F1                & Accuracy          & F1               & Accuracy          & F1               & Accuracy         & F1               & Accuracy           & F1                 \\ \midrule
OPT-6.7B                 & —               & —               & —               & —              & 36.9              & 27.9             & 37.9             & 28.5             & 18.8               & 14.3               \\
BLOOM-7B                 & 29.7              & 26.2              & 14.8              & 18.1             & 29.7              & 28.1             & 6.6              & 12.2             & 20.2               & 21.2               \\
LLaMA-7B                 & 31.8              & 29.6              & 22.3              & 24.9             & 36.8              & 28.6             & 35.3             & 31.4             & 31.6               & 28.6               \\ \midrule \midrule
Alpaca-7B                & 40.2              & 23.7              & 33.7              & 24.4             & 37.9              & 24.9             & 39.4             & 26.2             & 37.8               & 24.8               \\
Vicuna-7B                & 33.2              & 33.6              & 34.2              & 32.9             & 35.5              & 34.8             & 48.5             & 40.6             & 37.9               & 34.9               \\
Vicuna-13B               & 42.6              & 35.6              & 44.0              & 36.9             & 47.0              & 38.6             & \underline {47.0}       & 42.5             & 45.2               & 38.4               \\
ChatGLM-6B               & 37.4              & 31.0              & 36.5              & 31.7             & 41.6              & 37.9             & 42.9             & 37.5             & 39.6               & 34.5               \\
Flan-T5-11B              & 24.6              & 21.5              & 29.9              & 29.3             & 25.9              & 23.7             & 38.4             & 38.4             & 29.7               & 26.9               \\ \midrule \midrule
Text-Davinci-002         & {\underline {45.2}}        & 36.2              & {\underline{45.7}}        & 37.3             & 46.6              & 40.4             & 46.2             & 42.5             & {\underline {45.9}}         & 39.1               \\
Text-Davinci-003         & 42.8              & {\underline {41.4}}        & 43.1              & {\underline {42.1}}       & \textbf{48.8}     & {\underline {43.2}}       & 46.9             & {\underline {43.4}}       & 45.5               & {\underline {42.5}}         \\
GPT-3.5-Turbo            & \textbf{46.9}     & \textbf{44.3}     & \textbf{46.8}     & \textbf{44.4}    & {\underline {47.2}}        & \textbf{44.7}    & \textbf{47.1}    & \textbf{45.7}    & \textbf{47.0}      & \textbf{44.8}      \\ 
% \midrule
% Random Guess             & —                 & —                 & —                 & —                & —                 & —                & —                & —                & 33.3               & 29.8               \\ 
\bottomrule
\end{tabular}
}
\vspace{-5mm} 
\end{table}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\usepackage{wrapfig}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> pope.tex <==
\clearpage

\setlength{\tabcolsep}{8.5pt}
\vspace{-15pt}
\begin{table*}[t]
\centering
\caption{\textbf{Main results on POPE tasks.} We evaluate the POPE task accuracy of various MLLMs on the MSCOCO, A-OKVQA, and GQA datasets with LLaVa-1.5 under different decoding settings. \textbf{Regular} refers to the scenario where direct sampling is applied. \textbf{Vision}, \textbf{Language} and \textbf{Multimodal} refer to vision-only, language-only, and multimodal collaboration variants of \model.
The \textbf{bold} and the \underline{underlined} refer to the highest and second highest metrics under each setting, respectively. Each value is followed by the difference relative to regular setting.}
\label{tab:pope-results}
\vspace{0.30cm}

\begin{adjustbox}{width=1\linewidth}
\tiny
\begin{tabular}{p{0.7cm} p{0.7cm} ccccc cccc cccc ccc}
\toprule
\textbf{Dataset} & \textbf{Setting} & \textbf{Method} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} \\ \midrule
 & Random & Regular & 83.53 (0.00) & 92.12 (0.00) & 73.33 (0.00) & 81.66 (0.00) \\
 &  & VCD & 86.40 (2.87) & 94.68 (2.56) & 77.13 (3.80) & 85.01 (3.35) \\
 &  & OPERA & \textbf{89.20} (5.67) & 92.68 (0.56) & \textbf{85.26} (11.9) & \textbf{88.81} (7.15) \\
 &  & \textbf{Vision} & 86.46 (2.93) & \textbf{96.27} (4.15) & 75.86 (2.53) & 84.86 (3.20) \\
 &  & \textbf{Language} & 88.00 (4.47) & \underline{95.96} (3.84) & 79.33 (6.00) & 86.86 (5.20) \\
 &  & \textbf{Multimodal} & \underline{88.93} (5.40) & 95.20 (3.08) & \underline{82.00} (8.67) & \underline{88.10} (6.44) \\
\cmidrule(lr){2-7} 
\multirow{6}{*}{MSCOCO} & Popular & Regular & 81.10 (0.00) & 87.89 (0.00) & 72.13 (0.00) & 79.23 (0.00) \\
 &  & VCD & 83.53 (2.43) & 89.29 (1.40) & 76.20 (4.07) & 82.23 (3.00) \\
 &  & OPERA & 86.83 (5.73) & 88.24 (0.35) & 85.26 (13.1) & 86.62 (7.39) \\
 &  & \textbf{Vision} & 84.56 (3.46) & \underline{91.57} (3.68) & 76.13 (3.00) & 83.14 (3.91) \\
 &  & \textbf{Language} & \underline{87.03} (5.93) & \textbf{91.80} (3.91) & \underline{88.13} (16.0) & \underline{87.17} (7.94) \\
 &  & \textbf{Multimodal} & \textbf{87.13} (6.03) & 86.35 (1.46) & \textbf{88.20} (16.0) & \textbf{87.26} (8.03) \\
\cmidrule(lr){2-7} 
 & Adversarial & Regular & 78.63 (0.00) & 82.96 (0.00) & 72.06 (0.00) & 77.13 (0.00) \\
 &  & VCD & 81.10 (2.47) & 84.47 (1.51) & 76.20 (4.14) & 80.12 (3.99) \\
 &  & OPERA & 81.13 (2.50) & 78.79 (4.17) & \textbf{85.20} (13.1) & \underline{81.87} (4.74) \\
 &  & \textbf{Vision} & \underline{82.20} (3.57) & \underline{86.64} (3.68) & 76.13 (4.07) & 81.05 (3.92) \\
 &  & \textbf{Language} & 81.73 (3.10) & 86.28 (3.32) & 75.46 (3.40) & 80.51 (3.38) \\
 &  & \textbf{Multimodal} & \textbf{83.70} (5.07) & \textbf{87.69} (4.73) & \underline{78.40} (6.34) & \textbf{82.78} (5.65) \\
\cmidrule(lr){1-7} 
& Random & Regular & 84.03 (0.00) & 87.67 (0.00) & 79.20 (0.00) & 83.22 (0.00) \\
 &  & VCD & 85.90 (1.87) & 88.27 (0.60) & 82.80 (3.60) & 85.44 (2.22) \\
 &  & OPERA & \underline{88.23} (4.20) & 86.13 (1.54) & \textbf{91.13} (11.9) & 84.59 (1.37) \\
 &  & \textbf{Vision} & 87.66 (3.63) & \underline{90.24} (2.57) & 84.46 (5.26) & \underline{87.25} (4.03) \\
 &  & \textbf{Language} & 85.96 (1.93) & 89.75 (2.08) & 81.20 (2.00) & 85.26 (2.04) \\
 &  & \textbf{Multimodal} & \textbf{88.93} (4.90) & \textbf{91.89} (4.22) & \underline{85.40} (6.20) & \textbf{88.52} (5.30) \\
\cmidrule(lr){2-7} 
\multirow{6}{*}{A-OKVQA} & Popular & Regular & 80.23 (0.00) & 80.87 (0.00) & 79.20 (0.00) & 80.02 (0.00) \\
 &  & VCD & 81.96 (1.73) & 81.44 (0.57) & 82.80 (3.60) & 82.11 (2.09) \\
 &  & OPERA & 83.40 (3.17) & 78.92 (2.05) & \textbf{91.13} (11.9) & \underline{84.59} (4.57) \\
 &  & \textbf{Vision} & 84.03 (3.80) & 83.74 (2.87) & \underline{84.46} (5.26) & 84.10 (4.08) \\
 &  & \textbf{Language} & \textbf{85.96} (5.73) & \underline{89.75} (8.88) & 81.20 (2.00) & \textbf{85.26} (5.24) \\
 &  & \textbf{Multimodal} & \underline{85.70} (5.47) & \textbf{92.60} (11.7) & 77.60 (1.60) & 84.43 (4.41) \\
\cmidrule(lr){2-7} 
 & Adversarial & Regular & 74.26 (0.00) & 72.33 (0.00) & 78.60 (0.00) & 75.33 (0.00) \\
 &  & VCD & 76.10 (1.84) & 72.90 (0.57) & 83.06 (4.46) & 77.65 (2.32) \\
 &  & OPERA & 73.90 (0.36) & 67.77 (4.56) & \textbf{91.13} (12.5) & \textbf{84.59} (9.26) \\
 &  & \textbf{Vision} & 76.86 (2.60) & 73.43 (1.10) & 84.20 (5.60) & 78.44 (3.11)  \\
 &  & \textbf{Language} & \underline{77.43} (3.17) & \textbf{74.98} (2.65) & 82.33 (3.73) & 78.48 (3.15) \\
 &  & \textbf{Multimodal} & \textbf{77.86} (3.60) & \underline{74.41} (2.08) & \underline{84.93} (6.33) & \underline{79.32} (3.99) \\
\cmidrule(lr){1-7} 
 & Random & Regular & 83.60 (0.00) & 87.11 (0.00) & 78.86 (0.00) & 82.78 (0.00) \\
 &  & VCD & 85.86 (2.26) & 88.21 (1.10) & 82.80 (3.94) & 85.41 (2.63) \\
 &  & OPERA & \underline{88.50 (5.90)} & 85.45 (1.66) & \textbf{92.80} (13.9) & \textbf{88.90 (6.12)} \\
 &  & \textbf{Vision} & 87.40 (3.80) & \underline{90.53} (3.42) & 83.53 (4.67) & 86.89 (4.11) \\
 &  & \textbf{Language} & 86.56 (2.96) & 90.18 (3.07) & 82.06 (3.20) & 85.93 (3.15) \\
 &  & \textbf{Multimodal} & \textbf{88.50} (5.90) & \textbf{90.81} (3.70) & \underline{85.66} (6.80) & \underline{88.16} (5.38) \\
\cmidrule(lr){2-7} 
\multirow{6}{*}{GQA} & Popular & Regular & 77.86 (0.00) & 77.32 (0.00) & 78.86 (0.00) & 78.08 (0.00) \\
 &  & VCD & 79.06 (1.20) & 77.04 (0.28) & 82.80 (3.94) & 79.82 (1.74) \\
 &  & OPERA & 79.80 (1.94) & 73.65 (3.67) & \textbf{92.80} (13.9) & \underline{82.12} (4.04) \\
 &  & \textbf{Vision} & \underline{80.80} (2.94) & \underline{79.20} (1.88) & 83.53 (4.67) & 81.31 (3.23) \\
 &  & \textbf{Language} & 79.93 (2.07) & 78.70 (1.38) & 82.06 (3.20) & 80.35 (2.27) \\
 &  & \textbf{Multimodal} & \textbf{82.36} (4.50) & \textbf{80.36} (2.04) & \underline{85.66} (6.80) & \textbf{82.92} (4.84) \\
\cmidrule(lr){2-7} 
 & Adversarial & Regular & 75.16 (0.00) & 73.31 (0.00) & 79.13 (0.00) & 76.61 (0.00) \\
 &  & VCD & 76.33 (1.17) & 73.23 (0.08) & 83.00 (3.87) & 77.81 (1.20) \\
 &  & OPERA & 75.00 (0.16) & 68.43 (4.88) & \textbf{92.80} (13.6) & \underline{78.77} (2.16) \\
 &  & \textbf{Vision} & \underline{76.80} (1.64) & 73.43 (0.12) & 84.20 (5.07) & 78.44 (1.83) \\
 &  & \textbf{Language} & 76.60 (1.44) & \underline{74.21} (0.90) & 81.53 (2.40) & 77.70 (1.09) \\
 &  & \textbf{Multimodal} & \textbf{79.53} (4.37) & \textbf{76.49} (3.18) & \underline{85.26} (6.13) & \textbf{80.64} (3.03) \\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{5mm}
\end{table*}

\clearpage
